Coarse-to-Fine Dual Encoders are Better Frame Identification Learners

Frame identification aims to find semantic frames associated with target words in a sentence. Recent researches measure the similarity or matching score between targets and candidate frames by modeling frame definitions. However, they either lack sufficient representation learning of the definitions or face challenges in efficiently selecting the most suitable frame from over 1000 candidate frames. Moreover, commonly used lexicon filtering ($lf$) to obtain candidate frames for the target may ignore out-of-vocabulary targets and cause inadequate frame modeling. In this paper, we propose CoFFTEA, a $\underline{Co}$arse-to-$\underline{F}$ine $\underline{F}$rame and $\underline{T}$arget $\underline{E}$ncoders $\underline{A}$rchitecture. With contrastive learning and dual encoders, CoFFTEA efficiently and effectively models the alignment between frames and targets. By employing a coarse-to-fine curriculum learning procedure, CoFFTEA gradually learns to differentiate frames with varying degrees of similarity. Experimental results demonstrate that CoFFTEA outperforms previous models by 0.93 overall scores and 1.53 R@1 without $lf$. Further analysis suggests that CoFFTEA can better model the relationships between frame and frame, as well as target and target. The code for our approach is available at https://github.com/pkunlp-icler/COFFTEA.

==> main/abstract.tex <==
Frame identification aims to find semantic frames associated with target words in a sentence. Recent researches measure the similarity or matching score between targets and candidate frames by modeling frame definitions. However, they either lack sufficient representation learning of the definitions or face challenges in efficiently selecting the most suitable frame from over 1000 candidate frames. Moreover, commonly used lexicon filtering (\textit{lf}) to obtain candidate frames for the target may ignore out-of-vocabulary targets and cause inadequate frame modeling. In this paper, we propose \ours, a \uline{Co}arse-to-\uline{F}ine \uline{F}rame and \uline{T}arget \uline{E}ncoders \uline{A}rchitecture. With contrastive learning and dual encoders, \ours efficiently and effectively models the alignment between frames and targets. By employing a coarse-to-fine curriculum learning procedure, \ours gradually learns to differentiate frames with varying degrees of similarity. Experimental results demonstrate that \ours outperforms previous models by 0.93 overall scores and 1.53 R@1 without \textit{lf}. Further analysis suggests that \ours can better model the relationships between  frame and frame, as well as target and target. The code for our approach is available at \url{https://github.com/pkunlp-icler/COFFTEA}.
% Previous work xxx.
% In this paper, we  xxx metric learning xxx, propose a dual-encoder framework.
% CoFFTEA COarse-to-Fine Frame and Target Encoder Architecture

==> main/conclusion.tex <==
We propose \ours, and its dual encoder can effectively model the definitions with learnable frame encoder and efficiently calculate the similarity scores between a target and all frames. We also conclude that there exists a trade-off between training \textit{w/ lf} and \textit{w/o lf}, and achieves a comprehensive performance with a two stage learning process. Detailed analysis of the experiments further demonstrates that our two encoders are not limited to their alignment but can also discover other connections between frame and frame, as well as target and target.

==> main/experiment.tex <==
% experiment


% 1、dataset & baseline
Our experiments mainly cover three aspects:
\begin{itemize}
    \item Main experimental results on frame identification: We compare the performance of \ours with previous approaches both with lexicon filtering (\textit{\textbf{w/ lf}}) and without lexicon filtering (\textit{\textbf{w/o lf}}).
    \item Further ablation study: to demonstrate the contributions of the learnable frame encoder and Coarse-to-Fine learning to the performance of \ours.
    \item In-depth representation analysis: We delve into a deeper analysis to investigate how the frame and target encoder of \ours can better represent the alignment between frames and targets, as well as the relationships between frames and frames, targets and targets.
\end{itemize}

\begin{table*}[t]
\centering
\small
\begin{tabular}{lllll}
\toprule
\textbf{Models} & \multicolumn{4}{c}{\textbf{Predictions \textit{w/o lf} from rank 2 to 5 (Top-1 is Becoming)}} \\
\midrule
$\mathcal{L}_\mathcal{B}$ only$\dagger$  & Transition\_to\_a\_state & Undergo\_transformation & Change\_post\_state & Undergo\_change \\
$\mathcal{L}_\mathcal{C}$ only$\dagger$  & \textcolor{rred}{\textbf{Activity\_start}} & \textcolor{rred}{\textbf{Launch\_process}} & \textcolor{rred}{\textbf{Make\_acquaintance}} & \textcolor{rred}{\textbf{Meet\_specifications}} \\
% \ours & Undergo\_transformation & Transition\_to\_a\_state & Transition\_to\_a\_quality & \textcolor{rred}{\textbf{Process\_initial\_state}} \\
\bottomrule
\end{tabular}
\caption{Predictions in positions 2 to 5 of ``The children and families who come to Pleasant Run are given the opportunity to \textbf{become} happy''. \textcolor{rred}{\textbf{red}} means the frame is irrelevant to the gold frame \textbf{Becoming}.}
\label{tab:cmp}
\end{table*}

\subsection{Datasets}
We have introduced \ours on two FrameNet datasets: FN 1.5 and FN 1.7. FN 1.7 is an extensive version of FN 1.5, with more annotated sentences and more defined frames. Following \citet{swayamdipta2017frame, su-etal-2021-knowledge}, we spilt the full text into train, dev and test set, and further use exemplars in FrameNet as pretraining data like \citet{peng-etal-2018-learning, zheng-etal-2022-double, tamburini-2022-combining}. Table \ref{tab:data} shows the statistics of two datasets.

% 2、train & test setting
\subsection{Models}
We mainly compare \ours with representative previous methods from the different categories shown in Fig.~\ref{fig:model}: traditional representation learning based methods without definitions~\citep{hartmann-etal-2017-domain}, dual encoder architectures with frozen frame encoders (KGFI~\citeyearpar{su-etal-2021-knowledge}, \citet{tamburini-2022-combining}), and single fused encoder architectures (FIDO~\citeyearpar{jiang-riloff-2021-exploiting}).
% \textbf{KID} \citep{zheng-etal-2022-double} use the most relevant architecture to map the similarity between frames and targets. \textbf{FIDO} \citep{jiang-riloff-2021-exploiting} exploits the coherence between frames and targets through one context encoder. 

In order to conduct further ablation study and deeper analysis, we also implement two baselines represented as (a) and (b) in Fig~\ref{fig:model}: \textbf{Lookup Table} with random initialization and \textbf{Lookup Table initialized with definition representations}. The implementation details of previous methods, baselines, and \ours can be found in~\S\ref{appendix:models}.

% However, most of them focus on results using lexicon filtering, it is insufficient and unreasonable. Thus, we implement two additional baselines. One is \textbf{Bert-onehot}, uses a linear network to map discrete frames to a 768-dimension embedding. The other is \textbf{with frame embedding}, differs in using frame encoder encode frame definitions, which can be compared with previous work using contextualized frozen frame embeddings. Further, \textbf{with contrastive learning} replaces the optimization objective from Cross-Entropy to Contrastive-Learning, transfers a more smooth methdo to modeling relationship between one target to all frames.

% Obviously, our baselines can used to verify two things: namely the advantages of dual encoders and the better alignment of our optimization objective.

% 实验setting 要不要写
% \subsection{Experiment Setting}

% 3、empirical results  主表
\subsection{Main Results}





% \begin{table*}[h]
% \centering
% \small
% \begin{tabular}{lcccccccc}
% \toprule
%   & \multicolumn{4}{c}{\textbf{FN 1.5}}  & \multicolumn{4}{c}{\textbf{FN 1.7} }   \\
% % \cline{2-5} \cline{6-9}
% \cmidrule(r){2-2} \cmidrule(r){3-5}  \cmidrule(r){6-6} \cmidrule(r){7-9}
% \multirow{-2}{*}{\textbf{Models}}  & 
% \textbf{Acc(lf)}  & \textbf{R@1}  & \textbf{R@3}  &  \textbf{R@5}  &  \textbf{Acc(lf)}  & \textbf{R@1}  & \textbf{R@3}  &  \textbf{R@5}   \\
% \midrule
% \citet{hartmann-etal-2017-domain} & 87.63 & 77.49 & - & - & 83.00 & 76.10 & - & - \\
% \citet{peng-etal-2018-learning}$\dagger$  & 90.00 & - & - & - & 89.10 & - & - & -\\
% \citet{su2021knowledge} & 92.13 & 85.63 & - & - & 92.40 & 85.81 & 91.59 & 92.88  \\
% \citet{jiang-riloff-2021-exploiting} & 91.30 & - & - & - & 92.10 & - & - & - \\
% \citet{tamburini-2022-combining}$\dagger$  & \textbf{92.57}& - & - & - & 92.33 & - & - & -  \\
% % \multirow{-5}{*}{\textbf{FN 1.7}} & \ours &    & 
% %     &       &       &       &       \\
% % \midrule
% %   \multicolumn{9}{c}{\textbf{Baselines}}  \\
% \midrule
% Bert-onehot$\dagger$  & 88.60  & 78.48   &  86.74  &  88.16     & 89.02   & 78.75   &  87.43  &  88.71   \\
% with frame embedding$\dagger$ & 90.67  & 84.82  &  88.39  &  89.32     & 90.65  & 85.76  &  88.57  &  89.65    \\
% with contrastive learning$\dagger$ &  90.90   & 86.20  & 90.08  &  90.83   & 90.93  &  86.60  & 89.87  &  90.87   \\
% % Bert-onehot  & 89.63 & 81.19 &  87.42  &  88.23  & 89.41  & 81.41  &  86.92  &  87.90   \\
% % with frame embedding & 91.40 & 82.34   &  87.12  &  88.62   & 90.65  & 82.45  &  87.81  &  89.26    \\
% % with contrastive learning &  91.51 & 83.72  &  89.13  &  90.42  & 91.29 &  83.88 &  89.10  &  90.59   \\
% % \multirow{-5}{*}{\textbf{FN 1.5}} & \ours &                         &                         &       &       &       &  \\
% % \midrule
% %   \multicolumn{9}{c}{\textbf{Ours}}  \\
% \midrule
% % In-batch Learning  & 91.82  & 84.73   &  94.47  &  96.18 & 91.99  & 84.79  &  93.80  &  96.11  \\
% In-batch Learning  & 91.82  & 84.73   &  94.47  &  96.18 & 91.58  & 84.88  &  93.88  &  95.90  \\
% % In-batch Learning$^*$  & 87.96   & 67.59   &  79.04  &  83.94  & 90.65   & 85.30   &  \textbf{95.04}  &  \textbf{96.60} \\
% In-candidate Learning   & 92.50 &  76.51   &  87.35  &  91.01 & \textbf{92.70}  & 78.33  &  88.93  &  91.64  \\
% \textcolor{red}{In-batch Learning$\dagger$}  & 90.94     & 86.77  &  \textbf{95.14}  &  \textbf{96.79} & 91.36     & 87.38  & \textbf{95.29} & \textbf{96.77}  \\
% % In-batch Learning$\dagger$  & 90.94     & 86.77  &  \textbf{95.14}  &  \textbf{96.79} & 91.51  & 87.27  & \textbf{95.08} & \textbf{96.63}  \\
% \midrule
% \ours$\dagger$   & \textbf{92.55}  & \textbf{87.69} &  92.64  &  94.71 & 92.64  & \textbf{87.34}   &  92.91  &  94.29 \\
% \bottomrule
% \end{tabular}
% \caption{Frame identification accuracy on FrameNet test dataset. 'lf' and 'w/o lf' denote using lexicon filtering or not respectively, and Top-k further show performance without lexicon filtering. '$\dagger$' denote use exemplars as extra data for training, more detailed discussion on exemplars will be provided in ablation experiment}%'*' denotes only pretraining on exemplars, it will be proved in section ** that using exemplars can not consistently improve model performance. } 
% \label{tab:main}
% \end{table*}


To compare our model with previous approaches, as well as our baselines. We report the accuracy (\textbf{Acc}) when lexicon filtering is applied, recall at k (\textbf{R@$k$}) when no lexicon filtering is used (indicating whether the gold frame is ranked in the top $k$ based on similarity), and an \textbf{Overall} score (harmonic average of \textbf{Acc} and \textbf{R@1}).

The upper block of Table~\ref{tab:main} shows the performance of previous representative methods in frame identification. \ours achieves a performance gain of 0.93 overall scores (88.98 v.s. 89.91), primarily due to a 1.53 increase in R@1 scores (85.81 v.s. 87.34) in the \textit{\textbf{w/o lf}} setting. This improvement can be attributed to the use of a learnable frame encoder and two-stage learning, which enhance the effectiveness of \ours in modeling definitions. Compared to KGFI, \ours achieves comparable Acc \textit{\textbf{w/ lf}} (92.40 v.s. 92.64) and consistently performs better in R@$k$, which further demonstrates that through combining in-batch learning and in-candidate learning, \ours is able to select the appropriate frame from both candidates (\textit{\textbf{w/ lf}}) and all frames (\textit{\textbf{w/o lf}}).

Moreover, it is worth noting that some methods (marked $\dagger$) does not utilize exemplars as training data, while previous researches \citep{su-etal-2021-knowledge, zheng-etal-2022-double} believe that using exemplars for training improves accuracy. Further discussion about using exemplars can be found in~\S\ref{sec:ablation}.

In addition to representative methods in Table~\ref{tab:main}, there is a series of frame identification studies that solely focus on Acc \textit{\textbf{w/ lf}}. We report the results of \ours and more previous frame identification works in~\S\ref{appendix:amb}.

% Our strong baselines in the second part indicate that using contextualized frame embeddings is better than linear mapping, directly optimizing one target to all frames can not be better than optimizing one target to in-batch frames, which implies that our optimization objective is more suitable for frame identification.

% The Coarse-to-Fine Learning procedure is shown in the third part, In-batch Learning can directly get comparable result in without lexicon filtering setting, while In-candidate Learning can get even better performance on lexicon filtering setting. This is a reasonable phenomenon since these two phases concentrate on different level, In-batch is for modeling comprehensive alignment while In-candidate is for modeling fine-grained frame-target relation.
% For comparison, we also shows In-batch Learning result only using exemplars, which can not consistently improve model performance. Its effectiveness  will be discussed in ablation study.

% Our best model, \ours, get best performance on both settings, especially boost 2.06\% and  1.53\% on without lexicon filtering setting on FN 1.5 and FN 1.7 respectively.

% Obviously, few previous works care about the without lexicon filtering setting. However, to our best knowledge, it is more meaningful and challenging metric, so we further test the performance using top-k accuracy.



% 这个结果已经包含在主表里了 不需要再展示
% lexicon filtering result on FN1.5 + FN1.7


\subsection{Ablation Study}
\label{sec:ablation}



\paragraph{Frame Encoder} Can learnable frame encoder contribute to frame identification? As is shown in the middle block in Table~\ref{tab:main}, lookup table without definitions achieved relatively low overall scores (83.57). However, when we initialize the lookup table with the definitions encoded by the frozen encoder, the lookup table showed a significant improvement in R@1 \textit{w/o lf}, with an increase of 6.42 points (78.75 v.s. 85.17). This indicates that even without adjusting the parameters, the frozen encoder of PLMs is capable of modeling the definitions to some extent.

To further explore its impact, we apply in-batch learning to the lookup table with definitions. This additional step results in a further improvement of 1.96 points in R@1 w/o lf (85.17 v.s. 87.13). This suggests that in-batch learning reduces the number of negative samples, decreases the learning difficulty, and ultimately leads to better performance.

Comparing \ours to these lookup tables, we find that unfreezing the frame encoder allows for better modeling of fine-grained semantic differences, resulting in a significant increase of 1.70 points in accuracy \textit{w/ lf} (90.94 v.s. 92.64). This demonstrates the effectiveness of incorporating an unfrozen frame encoder to enhance the modeling of subtle semantic distinctions and improve the performance of the frame identification task.
\paragraph{Coarse-to-Fine Learning} The bottom block in Table~\ref{tab:main} demonstrates the trade-off between in-batch learning ($\mathcal{L}_\mathcal{B} $ only) and in-candidate learning ($\mathcal{L}_\mathcal{C} $ only). \textbf{$\mathcal{L}_\mathcal{B} $ only} achieves the highest R@1 (84.88) and \textbf{$\mathcal{L}_\mathcal{C} $ only} yields the highest Acc (92.70). However, the former approach does not excel at distinguishing fine-grained frames (91.58 Acc), while the latter approach even performs worse than the lookup table on R@1 \textit{w/o lf} (78.33 v.s. 78.75).

Table~\ref{tab:cmp} gives a specific example for comparison. Both methods can correctly predict the frame corresponding to the target \textit{become} in the given sentence. However, when looking at the predicted frames in positions 2 to 5, the frames predicted by in-batch learning show structural relationships with \textit{Becoming}, while the frames predicted by in-candidate learning have no connection to \textit{becoming}. This reflects that in-candidate learning cannot distinguishing frames sufficiently.

To address this issue, we train \ours with $\mathcal{L}_{\mathcal{B}}$ on exemplars and then train \ours with $\mathcal{L}_{\mathcal{C}}$ with train split, which is equivalent to performing coarse-grained pretraining on a large-scale corpus and then fine-tuning on a smaller dataset for domain adaptation at a finer granularity.

We also apply in-batch learning on both train and exemplar. Due to the lack of hard negatives, its performance on Acc \textit{w/ lf} is lower than \ours (91.36 v.s. 92.64).
\paragraph{Exemplars} Using exemplars as additional training data is a common practice~\citep{peng-etal-2018-learning, chen-etal-2021-joint,zheng-etal-2022-double}. Since in-batch learning benefits from larger-scale data (84.88 v.s. 87.38 in Table~\ref{tab:main}), we chose to use the larger set, exemplars for the first stage of in-batch learning. However, this makes our results not directly comparable to those of previous methods~\citep{su-etal-2021-knowledge} that only use the training set. However, more training data does not necessarily lead to improved performance. As shown in Table~\ref{tab:exem}, the performance of \citet{tamburini-2022-combining} and our lookup table baselines decreases after using exemplars, possibly due to a domain mismatch between the exemplars and the training set. However, our two-stage approach effectively utilizes both datasets to get an improvement of 0.31 Acc, providing a more appropriate way to utilize exemplars for future work.


\begin{table}
\centering
\small
\begin{tabular}{lccc}
\toprule
\textbf{Models} & \textbf{w/ exem.} & \textbf{w/o exem.} & $\Delta$  \\
\midrule
% KGFI             & -     & 92.40 & -     \\
% KID              & 91.70 & -     & -     \\
\citet{tamburini-2022-combining}          & 91.42 & 92.33 & -0.91 \\
\midrule
Lookup Table      & 89.02 & 89.41 & -0.39 \\
% Bert-frame       & 90.65 & 90.65 & 0.00  \\
% Bert-contrastive & 90.93 & 91.29 & -0.36 \\
$+$ \textit{init.} with Def       & 90.40 & 90.66 & -0.26 \\
$+\ \mathcal{L}_\mathcal{B}$ & 91.06 & 91.23 & -0.17 \\
\midrule
$\mathcal{L}_\mathcal{B}$ only & 91.36 & 91.58 & -0.22 \\
\midrule
\ours  & \textbf{92.55} & \textbf{92.24} & \textbf{0.31} \\
% diff             & 0.85  & -0.16 &      \\
\bottomrule
\end{tabular}
\caption{Training with extra exemplars does not increase the model performance. \ours can effectively utilize exemplars via two-stage learning.}
\label{tab:exem}
\end{table}

% + in-candidate frame padding ablation
% \begin{table}[]
% \centering
% \small
% \begin{tabular}{lcc}
% \toprule
% \textbf{Methods} & \textbf{Acc}             & \textbf{R@1}           \\
% \midrule
% in-candidate random         & 92.34          & 77.81          \\
% in-candidate sib            & \textbf{92.70} & \textbf{78.33} \\
% CoFFTEA random              & \textbf{92.75} & \textbf{87.62} \\
% CoFFTEA sib                 & 92.64          & 87.34          \\
% \bottomrule
% \end{tabular}
% \caption{in-candidate padding ablation}
% \end{table}


\begin{table}[t]
\small
\centering
\begin{tabular}{lccc}
\toprule

\textbf{Models} & \textbf{Acc} & \textbf{Acc w/ \texttt{[MASK]}} & $\Delta$\\
\midrule
% Lookup Table$\dagger$  & 89.41    & 79.83   & 9.58   \\
% maen frozen ce  e40            & 90.65    & 78.40   & 12.24  \\
% maen frozen scl e40            & 91.29    & 78.63   & 12.66  \\
% $+$ \textit{init.} with Def$\dagger$  & 90.66    & 80.43   & 10.23  \\
% $+$ Contrastive Loss$\dagger$  & 91.23  & 79.04  & 12.18  \\
Lookup Table   & 89.02    & 78.11   & 10.92  \\
% mean frozen train+exemplar ce  & 90.65    & 82.16   & 8.49   \\
% mean frozen train+exemplar scl & 90.93    & 77.82   & 13.11  \\
$+$ \textit{init.} with Def  & 90.30 & 77.58 & 12.72   \\
$+\ \mathcal{L}_\mathcal{B}$ & 90.94 & 77.91 & 13.03  \\
% \midrule
% $+\ \mathcal{L}_\mathcal{B}$$\dagger$ & 91.58    & 82.13   & 9.46   \\
% in-candidate lu+random         & 92.34    & 87.32   & 5.02   \\
% $+\ \mathcal{L}_\mathcal{C}$     & 92.70    & 86.91   & 5.79   \\
% from pretrian lu+random        & 92.75    & 86.34   & 6.40   \\
\midrule
\ours  & \textbf{92.64} &  \textbf{85.82}  & \textbf{6.82}  \\
\bottomrule
\end{tabular}
\caption{Masking target words can cause the decrease of accuracy. The extent of the decrease, $\Delta$, reflects whether the model understands the context information of the target.}
\label{tab:mask}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{lcccc}
\toprule
  &  & \multicolumn{3}{c}{\textbf{10 target exemplars}} \\
\cmidrule(r){3-5}
\multirow{-2}{*}{\textbf{Models}}  &  \multirow{-2}{*}{\textbf{R@1}}      & \textbf{R@1}      & \textbf{R@3}      & \textbf{R@5}      \\
\midrule
% Lookup Table$\dagger$ & 81.41 & 58.12 & 71.11 & 74.83    \\
% $+$ \textit{init.} with Def$\dagger$ & 81.96  & 69.85 & 85.75 & 88.43    \\
% $+$ Contrastive Loss$\dagger$ & 84.23  & 73.71 & 88.53 & 90.85    \\
Lookup Table   & 78.75 & 63.96    & 75.54    & 77.27    \\
$+$ \textit{init.} with Def & 85.17  & 81.71 & 89.51 & 90.33    \\
$+\ \mathcal{L}_{\mathcal{B}}$ & 87.13  & 83.04 & 92.24 & 93.40   \\
\midrule
% $+\ \mathcal{L}_\mathcal{B}$$\dagger$  & 84.88  & 70.35  & 89.02 & 93.19  \\
% $+\ \mathcal{L}_\mathcal{C}$$\dagger$  & 78.33  & 61.86    & 82.65    & 88.26    \\
% $\mathcal{L}_\mathcal{B}$ only & 87.38  &   84.24  & 95.20  &  96.89 \\
% \midrule
\ours   & \textbf{87.34}  & \textbf{85.58}    & \textbf{93.07}    & \textbf{94.89}    \\
\bottomrule
\end{tabular}
\caption{Representing frames with definitions and ten target exemplars. The target encoder of \ours can get similar and consistent representations of targets related to the same frame.}
\label{tab:tt}
\end{table}

\begin{table}[t]
\centering
\small
\begin{tabular}{lr}
\toprule
\textbf{Models}  &  \multicolumn{1}{c}{
\textbf{Average $\Delta \alpha / \alpha$}} \\
\midrule
% Lookup Table$\dagger$     & -0.349     \\
% $+$ \textit{init.} with Def$\dagger$   & 0.0457  \\
% $+$ Contrastive Loss$\dagger$  & 0.0472 \\
Lookup Table  & 0.158 \\
$+$ \textit{init.} with Def  & 0.012  \\
$+\ \mathcal{L}_\mathcal{B}$ &  0.070 \\
\midrule
$\mathcal{L}_\mathcal{B}$ only$\dagger$   &  56.290   \\
% $+\ \mathcal{L}_\mathcal{B}$  &  79.007 \\
% \midrule
$\mathcal{L}_\mathcal{C}$ only$\dagger$  & 6.494   \\
% $\mathcal{L}_\mathcal{C}$ only$\dagger$ w/o. sibling  &  4.066   \\
\midrule
\ours   & \textbf{121.816} \\
\ours w/o. sibling    & 34.907 \\
\bottomrule
\end{tabular}
\caption{The learnable frame encoder better models the structured information between frames. The perception of structure in \ours comes from the first stage of in-batch learning and the utilization of siblings as hard negatives.}
\label{tab:ff}
\end{table}

\subsection{Further Analysis}
\paragraph{Target-Frame Alignments} The results in Table~\ref{tab:main} demonstrate that \ours effectively models the alignment between targets and frames. However, we still want to explore whether the model's ability to predict a frame is due to its accurate modeling of the target's contextual information in the sentence or if there are other shortcuts involved. Moreover, if \ours can effectively model the context of the target, it can also be used to discover out-of-vocabulary targets. To investigate this, we replace the target in the sentence with the \texttt{[MASK]} token and compute the similarity between the masked target representation and frames. Table~\ref{tab:mask} shows that when the target is masked, the accuracy of the model decreases across the board. \ours achieves the smallest decrease in performance ($\Delta$), indicating the capability of our dual-encoder structure to effectively model the alignment between target context and frames. This capability also indicates that \ours can explore out-of-vocabulary targets.

\paragraph{Target-Target Relations} The target encoder ensure a close proximity between targets and their corresponding frames.
However, we believe that different sentences the target representations in different sentences, which activate the same frame, are supposed to exhibit a high degree of similarity. We select ten exemplars for each frame and replace frame representations with the mean representation (centroid) of these exemplars. In Table~\ref{tab:tt}, we compare two frame representations: directly encoding the definition and encoding ten exemplars. \ours achieves consistent and similar performance in both settings (87.34 and 85.58), reflecting the similarity between the target representations of the same frame and the final frame representation, as captured by our target encoder.

\paragraph{Frame-Frame Relations}
Due to the semantic relations defined by FrameNet between frames (such as \textit{inheritance}, \textit{using}, \textit{subframe}, etc.), frames are not isolated but rather interconnected with each other, forming structural relationships. For example, if \textit{receiving} inherits from \textit{getting}, their representations should be similar. Frame representations should reflect the structural relationships. To evaluate the degree of similarity between a subframe $f_{sub}$ and its superframe $f_{sup}$, we define a metric,
\begin{align}
    \alpha &= \frac{1}{|\mathcal{F}|} \cdot\sum_{f\in \mathcal{F}} \cos(f_{sub}, f) \\
   \Delta\alpha &= \cos{(f_{sub}, f_{sup}}) - \alpha
\end{align}
$\frac{\Delta\alpha}{\alpha}$ is a normalized evaluation reflecting how a subframe is close to its superframe compared to other frames. We report the average $\frac{\Delta\alpha}{\alpha}$ ($\alpha > 0$) of \textit{inheritance} pairs in Table~\ref{tab:ff}.

The baselines (the upper block) without a learnable frame encoder struggle to model the relationships between frames effectively. The distance between subframes and superframes is almost the same as that between other frames. However, using a learnable frame encoder greatly improves the similarity between subframes and superframes.

In-candidate learning, if used alone, tends to overly focus on differentiating frames with similar semantics, which actually decreases the similarity between them (6.494 v.s. 56.290). On the other hand, \ours effectively models the similarity between associated frames. This is mainly because we use two-stage learning and treat siblings as hard negative examples during training (34.907 v.s. 121.816), which indirectly enables the model to learn the connection between subframes and superframes.



% frame-frame:
% 1.lu2frame sim



% 2.frame2 sib frame
% \begin{table}[]
% \centering
% \small
% \begin{tabular}{lcc}
% \toprule
% &  \textbf{w/ exem.}  &  \textbf{w/o exem.}  \\
% \multirow{-2}{*}{\textbf{Models}}  &  $\Delta \alpha / \alpha$  &  $\Delta \alpha / \alpha$ \\
% \midrule
% Lookup Table     & 0.158  &  -0.349 \\
% $+$ \textit{init.} with Def$\dagger$   & 0.0119  & 0.0457  \\
% $+$ Contrastive Loss   &  0.0695  &  0.0472 \\
% \midrule
% $+\ \mathcal{L}_\mathcal{B}$  &  79.007  &  56.290  \\
% $+\ \mathcal{L}_\mathcal{C}$  &  6.494 &  -  \\
% $+\ \mathcal{L}_\mathcal{C}$ w/o. sibling & 4.066 & - \\
% \midrule
% \ours   & 121.816   & training \\
% \ours w/o. sibling    & 34.907 & 17.823  \\
% \bottomrule
% \end{tabular}
% \caption{sub-sup frame v.s. sub-the other frames}
% \end{table}

% 3.frame visual
% ...

% target-target:
% knn accuarcy
% to clarify that 
% \begin{table}[t]
% \centering
% \small
% \begin{tabular}{lcccc}
% \toprule
%   &  & \multicolumn{3}{c}{\textbf{KNN}} \\
% \cmidrule(r){3-5}
% \multirow{-2}{*}{\textbf{Models}}  &  \multirow{-2}{*}{\textbf{w/ lf.}}      & \textbf{R@1}      & \textbf{R@3}      & \textbf{R@5}      \\
% \midrule
% Lookup Table$\dagger$ & 81.41 & 58.12 & 71.11 & 74.83    \\
% $+$ \textit{init.} with Def$\dagger$ & 81.96  & 69.85 & 85.75 & 88.43    \\
% $+$ Contrastive Loss$\dagger$ & 84.23  & 73.71 & 88.53 & 90.85    \\
% Lookup Table   & 78.75 & 63.96    & 75.54    & 77.27    \\
% $+$ \textit{init.} with Def & 85.17  & 81.71 & 89.51 & 90.33    \\
% $+$ Contrastive Loss & 87.13  & 83.04 & 92.24 & 93.40   \\
% \midrule
% $+\ \mathcal{L}_\mathcal{B}$$\dagger$  & 84.88  & 70.35  & 89.02 & 93.19  \\
% $+\ \mathcal{L}_\mathcal{C}$$\dagger$  & 78.33  & 61.86    & 82.65    & 88.26    \\
% $+\ \mathcal{L}_\mathcal{B}$ & 87.38  &   84.24  & 95.20  &  96.89 \\
% \midrule
% \ours   & 87.34   & 85.58    & 93.07    & 94.89    \\
% \bottomrule
% \end{tabular}
% \caption{knn target 2 target}
% \end{table}



% without lexicon filtering result and top-k result
% \begin{table*}[h]
% \centering
% \small
% \begin{tabular}{cccccccc}
% \toprule
% \multicolumn{2}{c}{}  & \multicolumn{2}{c}{\textbf{Test}}  & \multicolumn{4}{c}{\textbf{Top-k} }   \\
% \cline{3-8}
% \multicolumn{2}{c}{\multirow{-2}{*}{\textbf{Models}}}  & 
% \textbf{All}  & \textbf{Amb}  & \textbf{Top-1}  &  \textbf{Top-2}  &  \textbf{Top-3}  &  \textbf{Top-5}  \\
% \midrule
% & Bert-onehot          &                         &                         &       &       &       &       \\
% & Bert-onehot          &                         &                         &       &       &       &       \\
% & Bert-frame           &                         &                         &       &       &       &       \\
% & Bert-frame           &     &      &       &       &       &       \\
% \multirow{-5}{*}{\textbf{FN 1.7}} & \ours &    & 
%     &       &       &       &       \\
% \midrule
% & Bert-onehot          &                         &                         &       &       &       &       \\
% & Bert-onehot          &                         &                         &       &       &       &       \\
% & Bert-frame           &                         &                         &       &       &       &       \\
% & Bert-frame           &                         &                         &       &       &       &       \\
% \multirow{-5}{*}{\textbf{FN 1.5}} & \ours &                         &                         &       &       &       &  \\
% \bottomrule
% \end{tabular}
% \caption{Frame identification accuracy with lexicon filtering on FrameNet test dataset, 'All' and 'Amb' denote testing on test data and ambiguous data respectively. '$\dagger$' denote use both train set and exemplars for training.} 
% \end{table*}

% model performance on wo lexicon filter, all and amb
% target-frame
% % without lexicon filtering result on FN1.5 + FN1.7
% \begin{table}[ht]  
% \centering
% \label{tab:wolf}  
% \begin{tabular}{lcccc}
% \toprule 
%     & \multicolumn{2}{c}{\textbf{FN 1.5}}      & \multicolumn{2}{c}{\textbf{FN 1.7}} \\
% \cmidrule{2-3}   \cmidrule{4-5}
% \textbf{Models} & \textbf{All} & \textbf{Amb} & \textbf{All} & \textbf{Amb} \\ 
% \midrule
% SimFrameId&  77.49  &  -   &  76.10  &  -  \\   
% KGFI& 85.63 & 80.07   &  85.81 & 80.66 \\
% \midrule
% Bert-onehot& 81.19 & 73.92  & 80.79 & 75.12   \\
% Bert-onehot$\dagger$& 78.48 & 69.00   & 78.75 & 71.07 \\
% Bert-frame& 82.34 & 76.55    & 82.45 & 76.37 \\
% Bert-frame$\dagger$ & 84.82 & 76.15   & 85.76 & 77.16   \\
% \midrule
% \ours  & \textbf{87.69}  &  ..   &  \textbf{87.34} & 81.18  \\
% \bottomrule
% \end{tabular}
% \caption{Frame identification accuracy without lexicon filtering on FrameNet test dataset, 'All' and 'Amb' denote testing on test data and ambiguous data respectively. '$\dagger$' denote use both train set and exemplars for training.} 
% \end{table}


% 4、Analytical results 六个分析表

==> main/introduction.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{emnlp2023-latex/image/example.pdf}
    \caption{An example of Frame Identification. The target word \textit{get} in the sentence is associated with frame \textbf{\textit{Board\_vehicle}}. \textbf{Lexicon filtering} (\textit{lf}) considers frames that can be evoked by \textbf{get.v} as candidates.}
    \label{fig:example}
\end{figure} 

%This paper is about frame identification.
%这部分主要是说现在的工作他们的缺陷，一定要点清楚，然后再show我们的优点和改进的方案。
% 两大类缺点： 1、只分类 没有提metric learning； 2、拟合 lexical filtering cheat
% frame knowledge 转移到这部分吧 然后task formulation只写FI
% Frame semantics (cite) associates the meanings of words with encyclopedia knowledge named frames. FrameNet (cite) defines more than 1,000 frames to represent different events, situations, relations and objects, which can be evoked by target words in texts. 
Frame Identification~\citep{gildea-jurafsky-2000-automatic, baker-etal-2007-semeval} aims to identify a semantic frame for the given target word in a sentence. The frames defined in FrameNet~\citep{baker-etal-1998-berkeley-framenet} are associated with word meanings as encyclopedia knowledge~\citep{fillmore1976frame}, which represent different events, situations, relations and objects. 
% 再加一句表示frame identification的作用
Identifying frames can contribute to extracting frame semantic structures from a sentence, and frame semantic structures can be utilized in downstream tasks, e.g., Information Extraction \citep{si2018frame}, Machine Reading Comprehension \citep{guo-etal-2020-incorporating}.

Previous researches in frame identification selects an appropriate frame for a target by modeling the similarity or matching score between the target and frames. Recent efforts are made to represent frames with definitions in FrameNet \citep{jiang-riloff-2021-exploiting, su-etal-2021-knowledge, tamburini-2022-combining, zheng2023query}. However, limited by the large scale of frames, these methods either struggle to effectively model definitions due to the use of a frozen frame encoder or cannot efficiently select appropriate frames from all frames due to the use of a single encoder architecture.

Fig.~\ref{fig:example} illustrates an example of frame identification. For the target word ``get'' in the sentence, we need to select its corresponding frame from over a thousand frames in FrameNet (\textbf{All}): \textbf{\textit{Board\_vehicle}} (A Traveller boards a Vehicle). Previous frame identification methods \citep{peng-etal-2018-learning, jiang-riloff-2021-exploiting} typically apply lexicon filtering (\textbf{\textit{lf}}) by selecting the frame from a set of candidate frames (\textbf{Candidates}) for the verb ``get'' (e.g., \textit{Arriving}, \textit{Getting}, \textit{Board\_vehicle}, etc.). \textit{lf} effectively improves the accuracy of frame identification. However, the manually defined lexicons is not possible to cover all the corresponding targets for frame, which hinders the extension of frame semantics to out-of-vocabulary target words. 

Furthermore, we observed that training \textbf{\textit{w/o lf}} (without \textit{lf}) poses challenges in distinguishing fine-grained differences among candidate frames. Conversely, training \textbf{\textit{w/ lf}} (with \textit{lf}) can lead to an increased distance between the gold frame and other candidates, making it difficult to distinguish the gold frame from irrelevant ones. Consequently, in this paper, our aim is to enhance our model's performance in both the \textit{w/ lf} and \textit{w/o lf} scenarios.
% Thus, it is rational to employ frame identification in Information Extraction, Text Summarization, and related fields to capture structured, coherent information, which facilitates a deeper understanding of semantics.

% 前人方法，metric learning，如何建模frame的表示是重点
% Previous researches in frame identification selects an appropriate frame for a target by modeling the similarity or matching score between the target and frames. Recent efforts are made to represent frames with definitions in FrameNet \citep{jiang-riloff-2021-exploiting, su2021knowledge, tamburini-2022-combining, zheng2023query}. However, limited by the large scale of frames, these methods either struggle to effectively model definitions due to the use of a frozen frame encoder or cannot efficiently select appropriate frames from all frames due to the use of a single encoder architecture.

% 加原因

% \citet{su2021knowledge, tamburini-2022-combining} employ two pre-trained transformer encoders to encode target words and frame definitions separately. However, due to the large number of candidate frames, the frame encoder is frozen during the training phase (i.e., its parameters will not be updated). As a result, the modeling of frame definitions is insufficient. 

% \citet{jiang-riloff-2021-exploiting, zheng2023query} encode sentence and frame definition pairs with one fused encoder, the \texttt{[CLS]} head of the transformer encoder is used to predict the matching score between target and frame. However, when we need to select the most suitable frame for a target from all frames in FrameNet, we would need to encode more than 1000 sentence-definition pairs, which can be computationally expensive.

In this paper, we propose \ours, a \textbf{\uline{Co}}arse-to-\textbf{\uline{F}}ine \textbf{\uline{F}}rame and \textbf{\uline{T}}arget \textbf{\uline{E}}ncoder \textbf{\uline{A}}rchitecture. By employing a dual encoder structure, we can effectively store the representations of all frames during inference, enabling us to efficiently compute the similarity between the target and all frames. Furthermore, considering the constraints imposed by the number of frames, we incorporate contrastive objectives to enhance the trainability of the frame encoder, consequently improving our ability to model definitions more accurately. Additionally, employing a distinct frame or target encoder allows us to map certain frames and targets to a vector space and utilize distance measures to depict their relationship.

% 实际上也是一种curriculum learning

% Training \textbf{\textit{w/o lf}} poses challenges in distinguishing fine-grained differences among candidate frames. Conversely, training \textbf{\textit{w/ lf}} can lead to an increased distance between the gold frame and other candidates, making it difficult to distinguish the gold frame from irrelevant ones. 
To address the trade-off between training \textit{w/ lf} and \textit{w/o lf}, we propose a two-stage learning procedure, referred to as coarse-to-fine learning.
In the first stage, we employ \textbf{in-batch learning}, using the gold frames of other instances within a batch as hard negative examples. This step helps the model learn to discern frames with distinct semantics. In the second stage, we adopt \textbf{in-candidate learning}, where we utilize other frames from the candidate set as negative samples. This enables the model to further refine its ability to recognize fine-grained semantic differences. With coarse-to-fine learning, \ours achieves a comprehensive performance in both scenarios of \textit{w/ lf} and \textit{w/o lf}.
  
Experiments show that \ours, compared to previous methods on two FrameNet datasets, achieves competitive accuracy \textit{w/ lf} and outperforms them by up to 1.53 points in R@1 \textit{w/o lf} and 0.93 overall scores considering both settings. Ablations also verify the contributions of the dual encoder structure and the two-stage learning process. Further analyses suggest that both the target encoder and frame encoder can effectively capture the target-target, and frame-frame relationships.

Our contributions can be summarized as follow:
\begin{enumerate}
    \item We propose \ours, a dual encoder architecture with coarse-to-fine contrastive objectives. \ours can effectively model frame definitions with learnable frame encoders and efficiently select the corresponding frame from over 1,000 frames.
    \item We conclude the trade-off between \textit{w/ lf} and \textit{w/o lf}, and emphasize the performance \textit{w/o lf} in the evaluation of frame identification. With two-stage learning, \ours achieves an overall score improvement of 0.93 on frame identification.
    \item Further in-depth analysis demonstrates that our frame and target encoders can better model the alignment between frame and target, as well as the relationships between target and target, frame and frame.
\end{enumerate}
% can achieve competitive accuracy \textit{w/ lf} and  separately get comparable or even better results in \textit{w/o lf} and \textit{w/ lf}, and \ours combines the advantages of both and outperforms previous models on \textbf{Overall} assessment by up to 1.29\% and 0.93\% for FN1.5 and FN1.7. And further experiments verify the effectiveness of our learnable frame encoder and coarse-to-fine learning procedure, and demonstrate the well alignment between frames and targets, as well as frames and frames, targets and targets.
% Metric learning methods were employed to encode frames from FrameNet and targets from sentences into the same vector space. While target representations can be directly encoded with abundant pre-trained language models, how to represent frames remains a challenge. 

% 最近的工作开始关注frame的建模，使用definition和framenet中的结构，KGFI采用双encoder，但是对于definition用bert做特征提取，encoder本身不可学习；

% 另一些工作利用了Frame Identification的lexicon filtering编码frame-definition pairs，即在知道target词的时候，我们可以根据它的lemma形式确定它候选的frames，这使得一个target候选的frames数量变少（1000+减到10个左右）。然而

%需要一个图，说明frame identification本身，也说明w/ lexicon filtering和w/o lexicon filtering的区别
% Recent efforts were made to represent frames with knowledge in FrameNet including frame definitions and FrameNet ontological structures.

% 引出我们的工作，两阶段 双encoder，target encoder + definition encoder，建模similarity。in-batch contrastive learning + in-candidate xxx 对应两个优点




% Previous researches in frame identification made efforts to adopt metric-learning based methods to represent targets and frames. By modeling similarities between a target and frames, methods such as KID and KGFI (cite) sought to integrate frame knowledge in advance to obtain appropriate frame representations while concentrating on optimizing target representation. Conversely, FIDO (cite) aimed to concatenate sentences and frame definitions, thereby implicitly learning coherence within the text.
% All of these methods revealed the importance of frame knowledge, And frame knowledge ...





% 除了方法上的不一样，我们还发现了frame identification这个任务存在的一些问题：1. lexicon filtering的问题；2. 层次化分类的问题（这个非常重要，没有的话可能文章立意要弱一点，最优先做这个实验）
% However, what they did is just a simple adapting of the target and its corresponding frames in the train set, they can not meet the demand of the real world since 

% 之前的关于FI的介绍
% Frame Identification is a key step in frame semantic paring process, and its primary goal is to recognize the underlying conceptual structure triggered by a lexical unit (target) and connect it to a pre-defined frame from a linguistic resource such as FrameNet. Usually a frame characterizes a particular situation, event, or object while a lexical unit may be polysemous and can evoke different frames in different contexts.

% As for FrameNet, it is a large-scale lexicon based on Frame Semantics theory which contains information about frames, their associated lexical units, and frame elements. Given a sentence here, to say frame, lu, fe, and its definitions.
% We call these rich information as "frame knowledge".
% The frame knowledge are as follows:
% \begin{itemize}
%     \item [1)]\textbf{frame definition}: frame definitions
%     \item [2)]\textbf{lexical unit}: lexical units
%     \item [3)]\textbf{frame relation}: frame relations
% \end{itemize}


% This approach to language understanding is inspired by Frame Semantics, a linguistic theory developed by Charles J. Fillmore in the 1970s and 1980s. Frame Semantics posits that people interpret and make sense of language based on their knowledge of various frames, which are activated by specific words or phrases in the text. Frame Semantic Parsing seeks to apply this theoretical framework to the automated analysis of text, enabling computers to better comprehend and process human language.





% three part:
% frame identification not a classification task, and infer with lexical filtering, 

% metric learning to model the task and want to get better performance in both settting
% motivated by
%在本文，我们采用metric learning对这个任务建模，将句子中的target和所有的frame编码在同一个语义空间
%我们希望学到的encoder无论在有/没有lexicon filering的情况下都可以取得好的表现
%但：1.如果训练的时候采用没有lexicon filtering的setting，那么模型可能只是拟合lexicon filtering（即知道一个词对应哪些frames），学不到细粒度的in-candidate的区别
%2. 如果训练的时候采用有lexicon filtering的setting。那么模型的frame encoder学的是有偏的
%这里再加个baseline，每个LU，我就选取它candidate里top-1的frame
%这里还有一个问题，对于多数target，它对应的frame也只有1个，这种情况下in-candidate也是学得不好的

% also, knn is used.
% 此外，我们认为frame之间不应该被当作离散的类别，学到的frame表示也应该体现本身的ontology结构；为此我们提出了一个新的设定

==> main/mainres.tex <==
\begin{table}[t]
\centering
\small
\begin{tabular}{lccccc}
\toprule
\textbf{Datasets} & \textbf{exemplar} & \textbf{train} & \textbf{dev}  & \textbf{test} & \textbf{$|\mathcal{F}|$}    \\
\midrule
FN 1.5 & 153946   & 16621 & 2284 & 4428 & 1019 \\
FN 1.7 & 192431   & 19391 & 2272 & 6714 & 1221 \\
\bottomrule
\end{tabular}
\caption{Statistics of FrameNet dataset}
\label{tab:data}
\end{table}

\begin{table*}[t]
\centering
\small
\begin{tabular}{lcccccccccc}
\toprule
  & \multicolumn{5}{c}{\textbf{FN 1.5}}  & \multicolumn{5}{c}{\textbf{FN 1.7} }   \\
% \cline{2-5} \cline{6-9}
\cmidrule(r){2-2} \cmidrule(r){3-5}  \cmidrule(r){6-6} \cmidrule(r){7-7} \cmidrule(r){8-10} \cmidrule(r){11-11}
\multirow{-2}{*}{\textbf{Models}}  & 
\textbf{Acc}  & \textbf{R@1}  & \textbf{R@3}  &  \textbf{R@5}  &  \textbf{Overall}  &  \textbf{Acc}  & \textbf{R@1}  & \textbf{R@3}  &  \textbf{R@5}  &  \textbf{Overall}   \\
\midrule
\citet{hartmann-etal-2017-domain}$\dagger$   & 87.63          & 77.49          & -              & -              & 82.25          & 83.00          & 76.10          & -              & -              & 79.40          \\
% \citet{peng-etal-2018-learning}$\dagger$  & 90.00          & -              & -              & -              & -              & 89.10          & -              & -              & -              & -              \\
KGFI~\citeyearpar{su-etal-2021-knowledge}$\dagger$   & 92.13          & 85.63          & -              & -              & 88.76          & 92.40          & 85.81          & 91.59          & 92.88          & 88.98          \\
FIDO~\citeyearpar{jiang-riloff-2021-exploiting}$\dagger$   & 91.30          & -              & -              & -              & -              & 92.10          & -              & -              & -              & -              \\
\citet{tamburini-2022-combining}  & \textbf{92.57} & -              & -              & -              & -              & 92.33          & -              & -              & -              & -              \\
\midrule

Lookup Table& 88.60          & 78.48          & 86.74          & 88.16          & 83.23          & 89.02          & 78.75          & 87.43          & 88.71          & 83.57          \\
% \textbf{\textbf{MLP with Def (frozen)}}  & 90.67          & 84.82          & 88.39          & 89.32          & 87.65          & 90.65          & 85.76          & 88.57          & 89.65          & 88.14          \\
$+$ \textit{init.} with Def  & 90.40 & 83.56 & 88.25 & 89.32 & 86.85 & 90.30 & 85.17 & 88.93 & 89.87 & 87.66 \\
% \textbf{\textbf{$+$Contrastive Loss}}  & 90.90          & 86.20          & 90.08          & 90.83          & 88.49          & 90.93          & 86.60          & 89.87          & 90.87          & 88.71          \\
$+\ \mathcal{L}_\mathcal{B}$  & 91.06 & 86.52 & 91.73 & 92.68 & 88.73 & 90.94 & 87.13 & 92.30 & 93.21 & 89.00          \\
\midrule
$\mathcal{L}_\mathcal{B}$ only$\dagger$   & 91.82          & 84.73          & 94.47          & 96.18          & 88.13          & 91.58          & 84.88          & 93.88          & 95.90          & 88.10          \\
$\mathcal{L}_\mathcal{C}$ only$\dagger$ & 92.50          & 76.51          & 87.35          & 91.01          & 83.75          & \textbf{92.70}          & 78.33          & 88.93          & 91.64          & 84.91              \\
$\mathcal{L}_\mathcal{B}$ only & 90.94          & 86.77          & \textbf{95.14} & \textbf{96.79} & 88.81          & 91.36          & \textbf{87.38} & \textbf{95.29} & \textbf{96.77} & 89.33          \\
\midrule
\ours  & 92.55 & \textbf{87.69} & 92.64          & 94.71          & \textbf{90.05} & 92.64 & 87.34          & 92.91          & 94.29          & \textbf{89.91}  \\
\bottomrule
\end{tabular}
\caption{Main results on FN1.5 and 1.7. \textbf{Acc} denotes accuracy \textbf{with} lexcion filtering and \textbf{R@$k$} denotes recall at $k$ \textbf{without} lexicion filtering. \textbf{Overall} represents the harmonic mean of \textbf{Acc} and \textbf{R@1}, reflecting the comprehensive capability of models. Through dual encoders and two-stage learning, \ours outperforms the previous methods (the topmost block) by at least 0.93 overall scores. Ablation study on dual encoders and two-stage learning is listed in the middle and bottom blocks (\S~\ref{sec:ablation}). $\dagger$ means the model does not trained with exemplar sentences.}
\label{tab:main}
\end{table*}

==> main/method.tex <==
% coarse-to-fine dual encoder
% xxxx
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{emnlp2023-latex/image/model.pdf}
    \caption{Comparison between \ours and other baselines. \textbf{(a)} and \textbf{(b)} both fine-tune a Lookup Table containing embeddings of frames with corss entropy loss. \textbf{(b)} uses a frozen frame encoder to initialize the table. \textbf{(c)} employs a single fused encoder to measure the probability of sentence and definition matching. For efficiency purposes, \ours (d) also adopts a dual-encoder structure and leverages contrastive loss to unfreeze the frame encoder.}
    \label{fig:model}
\end{figure*}

To model the alignment between frames and targets efficiently and effectively, in this paper, we propose \ours, a dual encoder architecture with two-stage contrastive objectives. We compare \ours with other baselines modeling frame definitions (\S~\ref{sec:architecture}). Specifically, to achieve better represent learning of definitions, the frame encoder of \ours is learnable during training. Moreover, in order to  make \ours gradually learn to differentiate frames with varying degrees of similarity. We introduce two-stage learning in~\S\ref{sec:train-process}.

%As illustrated in figure \ref{fig:model},
% Previous research has attempted to model the relationship between frames and targets by either precomputing the frame embedding or utilizing lexicon filtering, due to the limitations of their modeling approaches. Nevertheless, these methods seem overly simplistic and may lack the robustness necessary for establishing persuasive and comprehensive relationships between frames and targets in more complex scenarios.

% Our proposed \ours addresses this limitation by constructing dual encoders (Section \ref{sec:architecture}) and implementing a coarse-to-fine learning process (Section \ref{sec:train-process}), and facilitates a more exhaustive and nuanced understanding of the relationships.
% 先介绍architecture dual encoder
\subsection{Model Architecture} \label{sec:architecture}
% \subsection{CoFFTEA} \label{sec:architecture}
In Fig.~\ref{fig:model}, we compare the dual-encoder architecture of \ours with three categories of previous methods in frame identification: (a) no definition modeling \citep{hartmann-etal-2017-domain, zheng-etal-2022-double}, (b) target encoder and frozen frame encoder \citep{su-etal-2021-knowledge, tamburini-2022-combining}, and (c) single fused encoder \citep{jiang-riloff-2021-exploiting}. Limited by the number of frames in FrameNet, the dual encoder architecture with cross entropy loss (b) have to fix the parameters of the frame encoder while the single encoder architecture (c) have to train and infer under the \textit{w/ lf} setting. Therefore, we still use two encoders to separately encode the sentence with targets and frame definition, and employ contrastive learning to make the frame encoder trainable.

We follow \citet{su-etal-2021-knowledge, jiang-riloff-2021-exploiting, tamburini-2022-combining} to use PLMs~\citep{devlin-etal-2019-bert} as target encoder (\S\ref{sec:target_enc}) and frame encoder (\S\ref{sec:frame_enc}).

 % categorized previous methods on frame identification into three categories: no definition modeling 
% \ours includes two components: target encoder (section \ref{sec:target_enc}) and frame encoder (section \ref{sec:frame_enc}).
% Specifically, target encoder is designed to obtain contextualized representation of the target words, frame encoder is responsible for encoding frame definitions to acquire frame representation.
% % \newline

% Pre-trained language models (PLMs) have demonstrated remarkable effectiveness in natural language understanding tasks, largely due to their bi-/uni-directional processing, Transformer architecture, and extensive pre-training on large corpora. These models excel at capturing contextual information and semantic relationships within sentences, making them well-suited for our framework. In our paper, we leverage BERT as the backbone of our dual encoders to harness its powerful language understanding capabilities.

% As we known, BERT is an effective pre-trained model for natural language understanding tasks, owing to its bidirectional processing, Transformer architecture, and extensive pre-training on large corpora. Its ability to capture contextual information and semantic relationships within sentences makes it suitable for our framework, where we utilize BERT as the backbone of dual encoders.
\subsubsection{Target Encoder} \label{sec:target_enc}
The target encoder converts input sentence $S$ with $n$ tokens $w_1,\dots,w_n$ into contextualized representations ${h_1, \dots, h_n}$. The contextualized representation $t$ of target span $w_{t_s},\dots,w_{t_e}$ ($1 \leq t_s \leq t_e \leq n$) is the maxpooling of $h_{t_s}, \dots, h_{t_e}$~\citep{zheng2023query}.
% \begin{gather}
%     e_1, e_2, \dots, e_n = E_t(S)  \\
%     h_t = MaxPooling(e_i, e_{i+1}, \dots, e_j)
% \end{gather}
\begin{align}
h_1, \cdots, h_n &= \mathrm{Encoder}_t(w_1,\cdots, w_n)
\end{align}
\begin{align}
t &= \mathrm{MaxPooling}\left(h_{t_s}, \cdots, h_{t_e}\right)
\end{align}
With the target encoder, we capture the contextual information of the target sentence and the sufficient modeling of context can be used to find out-of-vocabulary targets. Our goal is to not only ensure a close proximity between the representations of the target and the frame but also to ensure that the target representations in different sentences, which activate the same frame, exhibit a high degree of similarity. 
% This approach allows us to effectively capture the semantic relationships between the target and the frame across various sentences, thereby enhancing our overall comprehension of their connection.
% This approach allows us to capture the most salient information of the target span in the sentence while maintaining a fixed-size representation for further processing.
\subsubsection{Frame Encoder} \label{sec:frame_enc}
% As frame knowledge encompasses rich information besides frame definition, \citet{su2021knowledge, jiang-riloff-2021-exploiting, zheng-etal-2022-double} incorporate not only frame definition but also lexical unit definition and frame relation.  Compared with them, our frame encode $E_f$ is solely designed to encode specific frame definition to convey its meaning. 

Taking \textit{Board\_vehicle} as \texttt{frame name} and its corresponding definition \textit{``A Traveller boards a Vehicle that they intend to use as a means of transportation either as a passenger or as a driver''} as \texttt{def}. Similarly, frame encoder converts $D = \texttt{frame name|def}$, denoted as $w'_1,\dots, w'_m$ into representations $h'_1,\dots,h'_m$. We follow \citet{reimers-gurevych-2019-sentence} to regard meanpooling of all tokens as frame representations $f$.
% 可以在appendix加一个关于cls和mean pooling的ablation

\begin{align}
h'_1, \cdots, h'_m &= \mathrm{Encoder}_f(w'_1, \cdots, w'_m) \\
% \end{equation}
% \begin{equation}
f &= \mathrm{MeanPooling}(h'_1, \cdots, h'_m)
\end{align}
% Moreover, inspired from \citet{jiang-riloff-2021-exploiting}, we observe that incorporating exemplars of the corresponding frame leads to improved performance compared to using definitions alone, which serve as additional context for better understanding the frame's semantics. Consequently, we concatenate the frame definition with relevant exemplars further, by doing so, we enable the model to learn more nuanced and comprehensive frame representations.

% Furthermore, drawing inspiration from \citet{jiang-riloff-2021-exploiting}, we note that integrating exemplars corresponding to a specific frame enhances performance in comparison to employing definitions exclusively, as they provide supplementary context for a more profound comprehension of the frame's semantics. As a result, we concatenate the frame definition with pertinent exemplars, thereby facilitating the model's ability to acquire more comprehensive frame representations.

Through the frame encoder, we encode frame definitions to represent frames. Similar to the target encoder, the frame encoder not only focuses on aligning frames with targets but is also intended to reflect the semantic relationships between frames themselves, such as \textit{Inheritance} \citep{su-etal-2021-knowledge, zheng-etal-2022-double}.

\begin{figure}[t]
    \centering
    \includegraphics[trim=5pt 0pt 28pt 0pt, clip, width=\columnwidth]{emnlp2023-latex/image/twostage.pdf}
    \caption{Coarse-to-Fine Learning of \ours. In-batch learning \textbf{(a)} is first applied with coarse-grained in-batch negative examples $\mathcal{B}$. In-candidate learning \textbf{(b)} is then employed to differentiate gold frame with hard negatives $\mathcal{C}$.}
    \label{fig:twostage}
\end{figure}

% 再分别介绍in-batch  in-candidate 以及joint learning
\subsection{Learning Process} \label{sec:train-process}

In order to capture the alignment between frames and targets, we aim to minimize the distance between the target and the gold frame (positive pair) while maximizing the distance between the target and other frames (negative pairs) during the training process. However, encoding such a large number of frames, which exceeds 1000, and updating the encoders with gradients for all of them becomes infeasible. Therefore, we need to sample a subset of frames as negative pairs. As discussed earlier, both training \textit{w/o lf} and \textit{w/ lf} have their limitations. To address this, we propose a two-stage learning process in Fig.~\ref{fig:twostage}.

We first employ in-batch learning (\S\ref{sec:in-batch}), where we treat the gold frames of other targets in the same batch as negative examples. This allows us to learn coarse-grained frame semantic differences.
Then we utilize in-candidate learning (\S\ref{sec:in-cand}), where we treat other frames in lexicon filter candidates as hard negatives. This step helps us refine the frame representations and capture fine-grained semantic distinctions

Specifically, we adopt cosine similarity $\cos(t, f) = \frac {t\cdot f} {\|t\|\cdot\|f\|}$ as distance metric and utilize contrastive learning to distinguish positive pairs from negative pairs. Let $\mathcal{L}_{\mathcal{B}}$ and $\mathcal{L}_{\mathcal{C}}$ denotes the contrastive loss of in-batch learning and in-candidate learning. The main difference between the two-stage learning lies in the construction of negative pairs $\mathcal{B}$ and $\mathcal{C}$.
\begin{align}
\mathcal{L}_{\mathcal{B}} &= - \log \frac{\exp\left(\cos(t, f^+) / \tau\right)}{\sum_{f\in \mathcal{B} \cup \{f^+\}}{\exp\left(\cos(t, f) / \tau\right)}}   \\ 
\mathcal{L}_{\mathcal{C}} &= - \log \frac{\exp\left(\cos(t, f^+) / \tau\right)}{\sum_{f\in \mathcal{C} \cup \{f^+\}}{\exp\left(\cos(t, f) / \tau\right)}}
\end{align}
% \begin{equation}
%     \cos(t, f) = \frac {t\cdot f} {\|t\|\cdot\|f\|}
% \end{equation}

% What is an optimal relationship between frames and targets? Ideally, the interrelationship amongst frames should embody the inherent connections defined by frame relations, while the associations between targets should exhibit strong correlations corresponding to belonging frames. Furthermore, the connection between a target and all frames ought to display a distinct hierarchy of closeness and similarity, reflecting frame relations simultaneously.

% However, \citet{su2021knowledge, zheng-etal-2022-double} use frame knowledge to get constant frame embeddings through frame encoder, \citet{jiang-riloff-2021-exploiting} assesses the suitability of a frame for a target word in a sentence based on the semantic coherence of their meanings. They are all necessitated by the constraints of their methods, unable to concurrently update the embeddings of all frames, or just structurally impossible to implement. Inevitably, they just construct a sub-optimal relationships, as it might not adequately capture the dynamic and evolving nature of the relationships between frames and targets,  force model to make potential compromises.
% Their decisions are necessitated by the constraints of their methods, which imply that concurrently updating the embeddings of all frames would entail significant computational expenses or just structurally impossible to implement. Inevitably, they seem to be somewhat limited in scope, as it might not adequately capture the dynamic and evolving nature of the relationships between frames and targets, potentially the model's overall effectiveness will be compromised.

% Therefore, we introduce \ours, a coarse-to-fine process to ascertain fine grained frame-to-target relations, respectively named In-batch Learning (section \ref{sec:in-batch}) and  In-candidate Learning  (section \ref{sec:in-cand}).

% In-batch Learning (section \ref{sec:in-batch}), utilizing contrastive learning to satisfy the co-relation between one target to all frames.

% Further, lexicon filtering reveals that one target maybe polysemous and naturally it would be hard to distinguish between the candidate frames. So the second stage In-candidate Learning  (section \ref{sec:in-cand}) proposes to optimize co-relation between target and its polysemous frames.


\subsubsection{In-batch Learning}   \label{sec:in-batch}
% 两件事情，既可以同时建模一个target和所有的frame  又可以保持更新，并且对比学习潜在地就会拉近相同类别，那么这个relation也是会有学习的
Training directly \textit{w/ lf} may cause the model to primarily focus on distinguishing the differences between the gold frame and the candidates. In order to broaden the model's horizons, we first conduct training \textit{w/o lf}, allowing the model to learn to differentiate coarse-grained semantic differences. We follow \citet{khosla2020supervised} to construct in-batch negative examples $\mathcal{B}$.
% Similar to dual-encoder architectures, incorporating a graph network within the frame encoder to encode ontological structure and optimizing through Cross-Entropy renders the updating of the frame encoder infeasible in \citet{su2021knowledge, zheng-etal-2022-double}. This is due to the requirement of encoding all frames at each step and updating the entire graph during each backward pass, thereby imposing considerable computational constraints on the model. Of course they can choose to only update the frame embeddings, but it doesn't make any sense or have any effect for optimizing frame encoder.
%  % 他们也可以选择将latent更新，但是这应该是没有意义的，因为肯定是更新encoder参数才会有作用

% Fortunately, leveraging Contrastive Learning in mini-batch enables the potential encoding of relationships between one target to all frames, while simultaneously allowing for the efficient updating of frame encoder with minimal computational cost.

% Specifically, for $\left( \mathbf{s}_i, \mathbf{f}_i \right)$ within a mini-batch $\mathcal{B}$, we  extract target representation $t_i$ and frame representation $f_i$ from dual encoders. The contrastive loss on the mini-batch $B$ is defined as:
% \begin{equation}
%     \ell_B(i) = \frac{\sum_{\substack{j \in C_i}}{\exp{\left(sim(t_i, f_j) / \tau \right)}}}
%     {{\sum_{\substack{k \in B}}}{ \exp{\left(sim(t_i, f_k) / \tau \right)}}}
% \end{equation}
% \begin{equation}
%     \mathcal{L}_B = \frac{1}{N_B} \sum_{i \in B} {
%     - \log \frac{1}{C_i} {\ell_{B}(i)}} 
%     % \mathcal{L}^{sup}_B = \sum_{i \in B}{ - \log \frac{1}{C_i} \sum_{\substack{f_i = f_c, c \neq i}}{P^{sup}_{B}(i, c)}}
% \end{equation}
% % \begin{equation}
% %     \ell_B(i, j) = \frac{\exp{\left(sim(t_i, f_j) / \tau \right)}}{
% %     {\sum_{\substack{k \in B}}}{ \exp{\left(sim(t_i, f_k) / \tau \right)}}}
% % \end{equation}
% % \begin{equation}
% %     \mathcal{L}_B = \frac{1}{N_B}\sum_{i \in B}{ - \log \frac{1}{C_i} \sum_{\substack{\mathbf{f}_i = \mathbf{f}_j, j \neq i}}
% %     {\ell_{B}(i, j)}} 
% %     % \mathcal{L}^{sup}_B = \sum_{i \in B}{ - \log \frac{1}{C_i} \sum_{\substack{f_i = f_c, c \neq i}}{P^{sup}_{B}(i, c)}}
% % \end{equation}
% % \frac{\mathbf{A} \cdot \mathbf{B}}{\|\mathbf{A}\|
% Here, $\ell_B(i)$ indicates the likelihood that $t_i$ is most similar to $f_i$ and $\tau$ is the temperature of Softmax. Ans we simply use 
% $sim(t_i, f_j) = \frac{t_i \cdot f_j}{\|t_i\|\|f_j\|}$ for similarity metric. The contrastive loss $\mathcal{L}_B$ is calculated for every sentence $\mathbf{s}_i$ among $B$, where $C_i = \left|\{c | \mathbf{f}_i = \mathbf{f}_j, j \neq i \}\right|$ is the number of samples in the same frame $\mathbf{f}_i$ in $B$.

% % 对比学习将所有的都视为负样本，其实是有偏的，但可以聚集各个frame
% Specifically, this approach inherently facilitates the alignment, since contrastive learning serves to draw closer targets belonging to the same frame and push targets from different frames further apart, thereby optimizing the learning of the desired relationships and enhancing the overall performance of the model in capturing a coarse alignment among frames and targets.
% materialize

\subsubsection{In-candidate Learning} \label{sec:in-cand}
\input{emnlp2023-latex/main/mainres}
Through in-batch learning, our model can effectively differentiate some frames that are relatively easy to distinguish. However, we aim to further distinguish frames that are more likely to be confused with one another. Typically, when using \textit{lf}, the other candidate frames for the same target can serve as negative examples $\mathcal{C}$.

However, the number of candidate frames for different targets can vary, and there are even cases where some targets only activate one frame in FrameNet. To address this issue, we pad the number of $\mathcal{C}$ for all targets to a fixed number (e.g., 15). This padding ensures that each target has a consistent number of candidate frames available for comparison during the training process.
% 为什么要使用in-candidate  1、因为in-batch将所有other frame视作负样本，使用小的t使得softmax的结果更加尖锐，但是进一步的还是可以去使用hard lu padding，以及使用sib去padding
% Simply treating all frames as negative samples will definitely introduce bias, as frame relations like $Inheritance$, $Using$, $Perspective\_on$ connect two frames with strong correlation.

We consider leveraging the semantic relationships between frames in FrameNet (\S\ref{appendix:relation}) to expand $\mathcal{C}$. \textit{Inheritance} represents the "is-a" relationship between frames. For example, \textit{receiving} inherits from \textit{getting}, then \textit{getting} becomes the super frame and \textit{receiving} becomes the sub frame. Other frames that also inherit from \textit{getting}, such as \textit{Commerce\_buy} and \textit{Taking}, are considered siblings of \textit{receiving}. These siblings exhibit semantic similarities with \textit{receiving}, but with subtle differences, making them suitable as hard negative examples. We follow the order of candidate frames, sibling frames, and random frames to construct $\mathcal{C}$.

% As FrameNet defined, a lexical unit may be polysemous and refers to multiple frames in different contexts, we call its corresponding frames as candidates. 
% What \citet{jiang-riloff-2021-exploiting} focus on is aligning this special frame-to-candidate relations. Moreover, frame relations like $Inheritance$, $Using$, $Perspective\_on$ always connect two frames with strong correlation. Obviously the above partial relations are hard to follow in our In-batch learning process, since we just treat all frames as equivalent negative frames.  So our In-candidate Learning try to figure it out and focus on the meticulous design of negative frames, especially the hard one, which plays a crucial role in the efficacy of contrastive learning approaches.
% % acknowledge that frames are inherently not completely independent.
% % 这里还需要再补充一个frame relation的图，去说明sibling的关系

% Undoubtedly, frames triggered by the same lexical unit is the first hard negatives, which represent the ability to capture contextual context. Second, frame relation itself contains a hierarchical structure, frames connected by $Inheritance$ introduce hallucinations and hard to distinguish. So we further seek the sibling frames as the second. Further, to capture the ability of In-batch Learning, we randomly choose a number of frames as negative frames. And this process can be defined in the following:
% \begin{equation}
%     \ell_{cand}(i) = \frac{\exp{\left(sim(t_i, f_i) / \tau \right)}}{
%     {\sum_{\substack{k \in cand}}}{ \exp{\left(sim(t_i, f_k) / \tau \right)}}}
% \end{equation}
% \begin{equation}
%     \mathcal{L}_B = \frac{1}{N_B}\sum_{i \in B}{ - \log \ell_{cand}(i)} 
%     % \mathcal{L}^{sup}_B = \sum_{i \in B}{ - \log \frac{1}{C_i} \sum_{\substack{f_i = f_c, c \neq i}}{P^{sup}_{B}(i, c)}}
% \end{equation}
% Here, $\ell_{cand}(i)$ indicates the likelihood that $t_i$ is most similar to $f_i$ over all negative frames and $\tau$ is the temperature of Softmax. Ans every sentence $\mathbf{s}_i$ among $B$ will calculate contrastive loss among $cand = \{f | f_{candidate}, f_{sibling}, f_{random} \}$.

% % Through In-candidate Learning, our model can capture a more fine-grained frame-to-target relations, and incorporate the hierarchical frame relation at the same time, which compensate In-batch Learning and form a good alignment between frames and targets.
% Through the implementation of In-candidate Learning, our model is capable of capturing more fine-grained frame-to-target relationships while simultaneously incorporating hierarchical frame relations. This approach compensates for the limitations of In-batch Learning and facilitates an optimal alignment between frames and targets.

% 不对 这并不是我的出发点，我的出发点是这一阶段可以区分lu pad和sib pad
% 所以他刚好可以作为in-batch的补充 这么说才会合理


% temp=1是为了不尖锐


==> main/relatedwork.tex <==
% 不要写得太细
% 可以看下AGED对FSRL的介绍  ok
% 突出重点！
\paragraph{Frame Identification}
Prior research in frame identification has primarily focused on modeling the similarity between targets and frames or assessing the matching score between them.

In terms of modeling similarity, \citet{hartmann-etal-2017-domain, peng-etal-2018-learning, zheng-etal-2022-double} leverage target encoder with a trainable frame representation table, while ignoring the valuable contextual frame information provided by FrameNet. To remedy this deficiency, \citet{su-etal-2021-knowledge, tamburini-2022-combining} both propose to incorporate frame definitions into frame encoder. Despite these efforts, the number of frames and the optimizing objective make it infeasible to update frame representation during training, leading to a compromise of freezing it. Consequently, they all trap in the dilemma to obtain optimal frame representation.
As for assessing the matching score, \citet{jiang-riloff-2021-exploiting} propose a fused encoder to evaluate semantic coherence between sentence and frame definition. Nevertheless, it just fails to evaluate the performance of \textit{w/o lf} scenario.

In addition, the aforementioned studies tend to adopt a one-sided relationship between targets and frames. They only train model on either \textit{w/ lf} or \textit{w/o lf}, which can not catch an overall horizon in distinguishing frames. Moreover, only \citet{su-etal-2021-knowledge} release performance under \textit{w/o lf} scenario, which is essential for evaluating the full capabilities of the model.

Some other work like \citet{Chanin2023OpensourceFS} treat frame semantic parsing as a sequence-to-sequence text generation task, but its still trap in training under \textit{w/ lf} and can not catch an optimal relationships.


\paragraph{Metric Learning} Metric learning is a fundamental approach in machine learning that seeks to learn a distance metric or similarity measure that accurately captures the inherent relationships between data points. One particular technique that has gained prominence in this area is Contrastive Learning, which has been extensively applied to a variety of tasks such as text classification \citep{gao-etal-2021-simcse}, image classification \citep{he2020momentum}. 

The optimized feature space retrieved from Contrastive Learning objective can benefit on learning better representations of data and capturing inner relationship. For frame identification, the primary goal is to obtain a well-aligned target-to-frame space. However, existing researches only focus on using Cross Entropy to directly modeling correlation to All Frames, which presents challenges in capturing complex relationships. Alternatively, Contrastive Learning can be leveraged to optimize and incrementally construct the feature space of frames and targets.

% Frame Identification is the first and core subtask of frame semantic parsing, it has attracted many researchers to make efforts since the SemEval 2007 shared task \citep{baker2007semeval}. 

% Generally, the objective of this subtask is to model the matching degree between the contextualized information of the target and the semantic information associated with the frame. Based on this, we can define the previous works as three paradigms:
% \begin{itemize}
%     \item \textbf{point-wise}: \citet{baker2007semeval, das-etal-2010-probabilistic, swayamdipta2017frame} treated it as a simple classification task, and only considered to learn the representation of the target through SVM, LSTM or other probabilistic models. This kind of learning is very one-sided and does not combine the characteristics of the task.
%     \item \textbf{pair-wise}: \citet{jiang-riloff-2021-exploiting} came to concatenate the frame and target in a pair-wise format, and accessed suitability based on the semantic coherence. However, a unified input can not satisfy w/o lexical filter test setting.
%     \item \textbf{decoupled}: \citet{su2021knowledge, zheng-etal-2022-double} proposed encoding the frame and target separately and incorporating frame knowledge into the frame encoder. What they aimed for was a better-aligned embedding space between frame and target. But they both failed due to the frame encoder being frozen during the training process.
% \end{itemize}

% In our method, we incorporate frame knowledge while training the two encoders jointly. Our focus is on learning a fine-grained alignment from easy to hard, which leads to better performance that more closely resembles real world scenarios.

% enhance // jointly  //disentangle

% old frame identification related work
%Previous works mainly relied on original sentence and its syntactic features. \citep{baker2007semeval, das-etal-2010-probabilistic, yang-mitchell-2017-joint, swayamdipta2017frame} treated frame identification as a simple classification task and predicted frames through SVM, LSTM or other probabilistic models. But considering such simple relationship between frame and target is one-sided. 
%And \citep{hermann-etal-2014-semantic, hartmann-etal-2017-domain} tried to map distributed representation of targets and frames into a common latent space. However, they all neglected the valuable frame knowledge annotated in FrameNet.

%Recently, \citep{su2021knowledge, jiang-riloff-2021-exploiting, zheng-etal-2022-double, zheng2023query, yamada2023semantic} started to use PLMS like BERT or T5 and proposed to incorporate frame knowledge into frame representation or contextualized target representation, but they either failed to establish fine-grained alignment or solely focused on simpler evaluation metric.

%Our method models the relationship between frames and targets from easy to hard, focuses on more comprehensive evaluation metrics, and shows better performance.

% \subsection{Metric Learning}
% Metric Learning focuses on learning distance metrics or similarity measures between data points in a feature space. Usually, Contrastive Learning is a specific technique used to achieve this goal, so that similar instances are close together and different instances are far apart. In the field of NLP, it plays a crucial role and has been applied in many tasks like text classification, information retrieval and machine translation \citep{gao2021simcse}, this optimized feature space can benefit on learning better representations of the textual data and capturing complex relationships between instances.

% Obviously, frame identification aims at learning the heterogeneous alignment between frames and targets, so metric learning can be utilized to optimize this goal, thus we use contrastive learning to progressively construct the feature space of frames and targets.

% \subsection{K-nearest neighbors}
% K-nearest neighbors (KNN) is a simple and efficient non-parametric algorithm used for classification and regression tasks. Recently, it has gained popularity again in the context of deep learning. %, particularly as a tool for training and evaluating deep neural networks.

% Researches often use KNN to evaluate the quality of learned representations in self-supervised learning like SimCLR \citep{chen2020simple}, or to classify new instances based on their similarity to the prototypes learned from Prototype Networks \citep{snell2017prototypical, liu2019prototype}.

% Since KNN is a versatile tool that can be used in various ways with deep neural networks, our work use KNN to not only help evaluate the quality of learned representations, 
% % but also be part of the model architecture to assist in classify the corresponding frames. (need to do soon)


%Frame Identification has attracted many researchers to make effort since the SemEval 2007 shared task \citep{baker2007semeval}. As the first and core subtask of frame semantic parsing, studying how to improve its performance is of great significance. 

%Most previous work only relied on original sentence and treated it as a classification task. \citep{johansson-nugues-2007-lth} proposed using SVM as a classifier and featured on a series of target information.\citep{das-etal-2010-probabilistic} utilized many syntactic features to a probabilistic model and predicted frame labels.

%However, since the frames of frame identification has much frames, some work try to model the relationship between target and frame.  

%However, since FrameNet has rich annotated information, researchers start to incorporate frame knowledge into frame identification and some work try to model the relationship between target and frame.
%\citep{hermann-etal-2014-semantic} presented a method using distributed representations of predicates and their syntactic context by mapping input representations and frame representations to a common latent space using the WSABIE algorithm (Weston et al., 2011). 
%\citep{hartmann-etal-2017-domain} implemented a model that jointly maps possible frame labels and the syntax context of target words into the same latent space using the WSABIE algorithm, and the syntax context was initialized with concatenating their word embeddings. 


==> main/taskformulation.tex <==
% \subsection{Frame Knowledge}

% frame definitions  and frame relations
% explain that each lu can evoke several frames are given, so it has two test setting,  give a equation.

For a sentence $S = w_1,\cdots,w_n$ with a target span $t = w_{t_s},\cdots,w_{t_e}$, frame identification is to select the most appropriate frame $f \in \mathcal{F}$ for $t$, where $\mathcal{F}$ denotes all frames in FrameNet.

% Directly, we can choosing appropriate frame from $\mathcal{F}$, and then \textbf{\textit{w/o lf}} can be formulated as follows:
% \begin{equation}  
% f_t = \arg\max_{f_i \in \mathcal{F}} P(f_i | t) 
% \end{equation} 

As FrameNet \citep{baker-etal-2007-semeval} provides each frame with an associated set of lexical units (LUs), we can obtain the LU of target $t$ by utilizing its lemma and part-of-speech (POS) in the form lemma.POS (e.g., \textbf{\textit{get.v}}) and apply  \textit{lf} to retrieve the lexicon filter candidate frames $\mathcal{F}_{t}$ of $t$. Then we focus on selecting $f \in \mathcal{F}_t$.
 

